Accelerating Reinforcement Learning Agent with EEG-based Implicit Human Feedback

Providing Reinforcement Learning (RL) agents with human feedback can dramatically improve various aspects of learning. However, previous methods require human observer to give inputs explicitly (e.g., press buttons, voice interface), burdening the human in the loop of RL agent's learning process. Further, it is sometimes difficult or impossible to obtain the explicit human advise (feedback), e.g., autonomous driving, disabled rehabilitation, etc. In this work, we investigate capturing human's intrinsic reactions as implicit (and natural) feedback through EEG in the form of error-related potentials (ErrP), providing a natural and direct way for humans to improve the RL agent learning. As such, the human intelligence can be integrated via implicit feedback with RL algorithms to accelerate the learning of RL agent. We develop three reasonably complex 2D discrete navigational games to experimentally evaluate the overall performance of the proposed work. Major contributions of our work are as follows, (i) we propose and experimentally validate the zero-shot learning of ErrPs, where the ErrPs can be learned for one game, and transferred to other unseen games, (ii) we propose a novel RL framework for integrating implicit human feedbacks via ErrPs with RL agent, improving the label efficiency and robustness to human mistakes, and (iii) compared to prior works, we scale the application of ErrPs to reasonably complex environments, and demonstrate the significance of our approach for accelerated learning through real user experiments.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section9.tex <==

\section{Appendix}
\label{sec:appendix}

% \begin{algorithm}[H]
% \caption{Riemannian Geometry based ErrP classification algorithm \citep{barachant2013classification}}

% \KwIn{Parameters $N_E, N_T$, acquisition function $a(\cdot)$}
% Initialize DQN $\mathcal{Q}(\cdot, \cdot)$ \;
% \For {episode=1,2,\ldots}{
% Starting from randomly selected initial state, the RL agent play the game until the end \;
% Update the DQN $\mathcal{Q}$ by experiences randomly selected from the replay buffer \;
% }
% \end{algorithm}
% \subsection{ErrP Decoding Algorithm}




%The network consists of a shared architecture with K bootstrapped "heads" branching off independently. Each head is trained only on its bootstrapped sub-sample of the data and represents a single bootstrap sample.The shared network learns a joint feature representation across all the data, which can provide significant computational advantages at the cost of lower diversity between heads. This type of bootstrap can be trained efficiently in a single forward/backward pass; it can be thought of as a data-dependent dropout, where the dropout mask for each head is fixed for each data point.

%\subsection{Acquisition Function}
%\label{sec:acq}
%In this work, three acquisition functions are explored in selecting trajectory for ErrP labeling. The trajectory is defined as a sequence of state-action pairs $\tau:=\{(\bm{s}_0, \bm{a}_0),\ldots,(\bm{s}_T, \bm{a}_T)\}$. We denote the trajectory set as $\mathcal{D}$, the learned Q network as $\mathcal{Q}$, and acquisition function as $a(\tau, \mathcal{Q})$. The selected trajectory maximizes the acquisition function given $\mathcal{Q}$. In this work, we explore three acquisition functions:
%\begin{itemize}
%\item {\it Entropy}: Select the trajectory with the maximum entropy, which measures the uncertainty of state-action pairs along the trajectory.
%\begin{equation}
%a(\tau, \mathcal{Q}):=\mathbb{H}[\tau|\mathcal{Q}]=-\sum_{t=0}^T \mathbb{H}[\bm{s}_t, \bm{a}_t|\mathcal{Q}] \nonumber
%\end{equation}
% Specifically, in Bayesian and bootstrapped DQN, since Q value is approximately Gaussian distributed, we can directly use the differential entropy of Gaussian random variable here, i.e., $\mathbb{H}[\bm{s}_t, \bm{a}_t|\mathcal{Q}]=\frac{1}{2}\log2\pi e\text{Cov}_a$, where the variance term $\text{Cov}_a$ can be replaced by \eqref{post} or the variance of $K$ heads of bootstrapped DQN. 
%\item {\it Mutual Information}: choose the trajectory with maximum mutual information between priors and posterior of state-action distributions \citep{houlsby2011bayesian}. The mutual information represents the information gain of action selections. We have
%\begin{equation}
%a(\tau,\mathcal{Q}):=\mathbb{I}[\tau|\mathcal{Q}]=\sum_{t=0}^T\mathbb{I}[\bm{s}_t,\bm{a}_t|\mathcal{Q}] \nonumber
%\end{equation}
%Following \citep{nikolov2018information}, we approximate the mutual information $\mathbb{I}[\bm{s}_t,\bm{a}_t|\mathcal{Q}]$ by $\log(1+\frac{\sigma(\bm{s}_t, \bm{a}_t)^2}{\rho(\bm{s}_t, \bm{a}_t)^2})$, where $\sigma(\bm{s}_t, \bm{a}_t)$ characterizes the {\it parametric uncertainty} of Q value, and $\rho(\bm{s}_t, \bm{a}_t)^2$ represents the {\it intrinsic uncertainty}. In this work, $\sigma(\cdot, \cdot)^2$ is obtained by $\text{Cov}_a$ in \eqref{post} for Bayesian DQN, and by the variance of $K$ heads in bootstrapped DQN. We approximate $\rho(\bm{s}_t,\bm{a}_t)$ by the variance of accumulated rewards $Z(\bm{s}_t,\bm{a}_t)$, obtained by histogram statistics, C51 \citep{bellemare2017distributional} or QR-DQN \citep{dabney2018distributional}.
%\item {\it Confidence Interval}: Choose the trajectory with the maximum uncertainty in ErrP labeling. Some state-action pairs may have ambiguous results of ErrP decoding, with similar numbers of true and false results. And taking these pairs for ErrP labeling can decrease the uncertainty, making the RL agent more decisive on action selection. Confidence level of Binomial random variable is used here as the metric of uncertainty. Then acquisition function based on confidence interval can be expressed as
%\begin{equation}
%\sum_{t=1}^T\frac{1.96}{N^s_t + N^f_t}\sqrt{\frac{N^s_tN^f_t}{N^s_t + N^f_t}}\nonumber
%\end{equation}
%where $N^s_t$ ($N^f_t$) are number of True (False) ErrP decoding results for state-action pair at step $t$ on the trajectory.
%\end{itemize}

\subsection{Reward Learning}
\label{sec:reward}
Since implicit human feedback via ErrP is noisy (hence \textit{imperfect demonstrations}), we model the reward learning as a probabilistic maximum entropy RL problem. Following the principle of maximum entropy, given Q function $Q(\cdot,\cdot)$, the policy distribution and value function in terms of Q function can be expressed as follows, 
\begin{eqnarray}
V_Q(\bm{s})&=&\alpha\log\sum_a\exp(Q(\bm{s},\bm{a})/\alpha), \nonumber \\ \pi_Q(\bm{a}|\bm{s})&=&\exp((Q(\bm{s},\bm{a})-V_Q(\bm{s}))/\alpha) \label{maxent}
\end{eqnarray}
where $\alpha$ is a free parameter, tuned empirically. The likelihood of positive and negative state-action pair are denoted as $\pi_Q(\bm{a}|\bm{s})$ and $1-\pi_Q(\bm{a}|\bm{s})$. When demonstrations and corresponding implicit human feedback are ready, we train the Q function by maximizing the likelihood of both positive and negative state-action pairs in the demonstrations. 

In order to refine the reward shape and attenuate the variance of learning updates, we introduce another baseline function $t(\bm{s})$ in the Q function. Hence, the Q function becomes $Q_B(\bm{s},\bm{a}):=Q(\bm{s},\bm{a})-t(\bm{s})$. It can be proved that $Q_B(\cdot,\cdot)$ and $Q(\cdot,\cdot)$ induce the same optimal policy \citep{ng1999policy}. The baseline function $t^*(\cdot)$ can be learned by optimizing $t^*=\arg\min_{t}J(t)$, and the objective is defined as
\begin{eqnarray}
J(t)&:=&\arg\min_{t}\sum_{(\bm{s}, \bm{a}, \bm{s}')\in\mathcal{D}\cup\mathcal{D}_R}l(Q(\bm{s},\bm{a})-t(\bm{s}) \nonumber \\ &&-\gamma\max_{\bm{a}'\in\mathcal{A}}(Q(\bm{s}',\bm{a}')-t(\bm{s}'))) \nonumber
\end{eqnarray}
where the loss function $l(\cdot)$ is chosen to be $l_1$-norm through empirical evaluations. In addition to the demonstration $\mathcal{D}$, we incorporate another set of demonstrations $\mathcal{D}_R$, containing transitions randomly sampled from environment without reward information. The set $\mathcal{D}_R$ is to help the function $t(\cdot)$ to efficiently learn the state dynamics, and does not require human labeling, essentially keeping the number of queries same. After reward learning, consisting of learning Q function and baseline function, for any transition tuple $(\bm{s}, \bm{a}, \bm{s}')$, the learned reward function can be represented as $Q_B(\bm{s}, \bm{a})-\gamma\max_{\bm{a}'\in\mathcal{A}}Q_B(\bm{s}',\bm{a}')$. We then use this reward function to augment the following RL agent. 


%\subsection{Box World Game Environment}
%\label{sec:box}
%This environment consists of an $8\times8$ pixels room with keys and boxes randomly scattered. The room also contains an agent, represented by a single black pixel, which can move in four directions: up, down, left, and right. Keys are represented by a single colored pixel, and boxes are represented by two adjacent colored pixels, where the pixel on the right represents the box's lock. A key can open a lock if it’s color matches the lock. Its screen shot is shown in Figure \ref{fig:box_sim} (a).
%\subsubsection{Evaluation with Synthetic Human Feedback}
%\label{sec:box_evaluation}
%Here, we evaluate the first framework on the Box World game \citep{zambaldi2018relational} with synthetic human feedback. This environment is introduced with details in Appendix \ref{sec:box}. The synthetic feedback gives noisy label on each state-action pair, where the correct (optimal) one is labeled as wrong (sub-optimal) with the probability of $\epsilon_1$, and the wrong (sub-optimal) one is labeled as correct with the probability of $\epsilon_2$. Here, the Q network is modeled by bootstrapped DQN.
%
%This game has a combinatorially complex environment which cannot be quickly solved by a regular RL algorithm. The simulation results are shown in Figure \ref{fig:box_sim}, where "No Feedback" refers to the RL algorithms without the help of human feedback. The detailed statistics of evaluations are illustrated in Table \ref{tab:box}. Three acquisition functions are evaluated for comparison. The mean complete episode for mutual information, entropy and confidence level are $167.0, 177.5$ and $231.2$ for Human 1, $166.3, 184.2$ and $195.2$ for Human 2. We can see the first framework can achieve similar performance as full access method in terms of convergence speed, with much smaller number of inquiries. The acquisition function of confidence interval performs worst, because it does not consider the properties of the trained model. The mutual information performs better than entropy, but needs a larger number of human feedback inquiries.
%
%\begin{figure}[ht]
%\centering
%\subfigure[Game Screen]{
%\begin{minipage}[t]{0.31\linewidth}
%\centering
%\includegraphics[width=1.1in]{box.pdf}
%\end{minipage}
%}
%\subfigure[Human 1]{
%\begin{minipage}[t]{0.31\linewidth}
%\centering
%\includegraphics[width=1.65in]{box_boot_sim2.pdf}
%\end{minipage}
%}
%\subfigure[Human 2]{
%\begin{minipage}[t]{0.31\linewidth}
%\centering
%\includegraphics[width=1.65in]{box_boot.pdf}
%\end{minipage}
%}
%\caption{First Framework Evaluation on Box World Game. The number in brackets denotes the inquiry interval $N_E$.}
%\label{fig:box_sim}
%\end{figure}
%
%
%\begin{table}[H]
%\label{tab:box}
%\centering
%\caption{First Framework Evaluation on Box World Game with Synthesized Human ($N_E$: Inquiry Interval $N_C$: Complete Episode $N_I$: Number of Inquiries). Standard deviation is presented in the brackets.}
%\setlength{\tabcolsep}{1.5mm}{\tiny
%\begin{tabular}{cc|cc|cc|cc|cc}
%\toprule
%\multirow{2}*{Human} & \multirow{2}*{$N_E$} & \multicolumn{2}{c}{Full Access} & \multicolumn{2}{c}{Mutual Information} & \multicolumn{2}{c}{Entropy} & \multicolumn{2}{c}{Confidence Interval} \\
% & & $N_{C}$ & $N_{I}$ & $N_{C}$ & $N_{I}$ & $N_{C}$ & $N_{I}$ & $N_{C}$ & $N_{I}$  \\\midrule
%$\epsilon_1=0.3, \epsilon_2=0.25$ & 5 & $166.9(36.2)$ & $7219.6(1236.0)$ & $167.0 (36.1)$ & 1010.3(208.2) & 177.3(31.8) & 758.9(298.4) & 231.2(26.2) & 1003.2(154.62) \\
%$\epsilon_1=0.2, \epsilon_2=0.15$ & 10 & 153.2(29.7) & 4562.2(325.3) & 166.3(33.0) & 743.3(117.5) & 184.2(61.9) & 510.6(165.3) & 195.2(30.0) & 809.9(154.6) \\
%\bottomrule
%\end{tabular}}
%\end{table}
%
%\begin{table}[H]
%\label{tab:maze}
%\centering
%\caption{First Framework Evaluation on Maze Game with Real ErrP}
%\setlength{\tabcolsep}{1.5mm}{\tiny
%\begin{tabular}{cc|cc|cc|cc|cc}
%\toprule
%\multirow{2}*{Subject} & \multirow{2}*{$N_E$} & \multicolumn{2}{c}{Full Access} & \multicolumn{2}{c}{Mutual Information} & \multicolumn{2}{c}{Entropy} & \multicolumn{2}{c}{Confidence Level} \\
% & & $N_{C}$ & $N_{I}$ & $N_{C}$ & $N_{I}$ & $N_{C}$ & $N_{I}$ & $N_{C}$ & $N_{I}$  \\\midrule
%Subject 04 & 5 & 153.4($\pm$27.8) & 1975.4($\pm$346.2) & 161.2($\pm$21.7) & 636.7($\pm$170.3) & 172.0($\pm$47.8) & 389.3($\pm$149.9) & 168.3($\pm$22.6) & 847.2($\pm$135.2) \\
%Subject 05 & 5 & 150.0($\pm$20.4) & 2130.1($\pm$357.8) & 153.1($\pm$36.8) & 505.7($\pm$221.6) & 164.8($\pm$25.4) & 394.7($\pm$109.1) & 173.8($\pm$39.6) & 887.1($\pm$292.0) \\
%\bottomrule
%\end{tabular}}
%\end{table}



